Inverse Problems Leveraging Pre-trained Contrastive Representations

We study a new family of inverse problems for recovering representations of corrupted data. We assume access to a pre-trained representation learning network R(x) that operates on clean images, like CLIP. The problem is to recover the representation of an image R(x), if we are only given a corrupted version A(x), for some known forward operator A. We propose a supervised inversion method that uses a contrastive objective to obtain excellent representations for highly corrupted images. Using a linear probe on our robust representations, we achieve a higher accuracy than end-to-end supervised baselines when classifying images with various types of distortions, including blurring, additive noise, and random pixel masking. We evaluate on a subset of ImageNet and observe that our method is robust to varying levels of distortion. Our method outperforms end-to-end baselines even with a fraction of the labeled data in a wide range of forward operators.

==> tex/tables_tex/10percent.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Linear probe with 10\% labels.} Here, the linear probe for each of the previously mentioned models is trained using only 10\% of the labeled samples. The supervised baseline is still trained with all labeled samples.}
\label{tab:10percent}
\begin{tabular}{lcc}
\toprule
Distortion                    & \begin{tabular}[c]{@{}c@{}}Supervised\\ Baseline\end{tabular} & Ours                  \\ \midrule
Random Mask 50\%              & 77.53$\pm$0.06                                                  & \textbf{82.19$\pm$0.08} \\
Random Mask 75\%              & 75.68$\pm$0.06                                                  & \textbf{80.36$\pm$0.09} \\
Random Mask 90\%              & 74.12$\pm$0.09                                                  & \textbf{79.87$\pm$0.12} \\
Gaussian Noise $\sigma$ = 0.1 & \textbf{82.23$\pm$0.04}                                         & 80.99$\pm$0.09          \\
Gaussian Noise $\sigma$ = 0.3 & 75.78$\pm$0.08                                                  & \textbf{78.16$\pm$0.07} \\
Gaussian Noise $\sigma$ = 0.5 & 71.43$\pm$0.14                                                  & \textbf{73.14$\pm$0.08} \\
Gaussian Blur n = 21          & 76.4                                                          & \textbf{80.94}        \\
Gaussian Blur n = 37          & 68.94                                                         & \textbf{74.84}        \\ \bottomrule
\end{tabular}
\end{table}
